Multi-Camera Calibration Free BEV Representation for 3D Object Detection

In advanced paradigms of autonomous driving, learning Bird's Eye View (BEV) representation from surrounding views is crucial for multi-task framework. However, existing methods based on depth estimation or camera-driven attention are not stable to obtain transformation under noisy camera parameters, mainly with two challenges, accurate depth prediction and calibration. In this work, we present a completely Multi-Camera Calibration Free Transformer (CFT) for robust BEV representation, which focuses on exploring implicit mapping, not relied on camera intrinsics and extrinsics. To guide better feature learning from image views to BEV, CFT mines potential 3D information in BEV via our designed position-aware enhancement (PA). Instead of camera-driven point-wise or global transformation, for interaction within more effective region and lower computation cost, we propose a view-aware attention which also reduces redundant computation and promotes converge. CFT achieves 49.7% NDS on the nuScenes detection task leaderboard, which is the first work removing camera parameters, comparable to other geometry-guided methods. Without temporal input and other modal information, CFT achieves second highest performance with a smaller image input 1600 * 640. Thanks to view-attention variant, CFT reduces memory and transformer FLOPs for vanilla attention by about 12% and 60%, respectively, with improved NDS by 1.0%. Moreover, its natural robustness to noisy camera parameters makes CFT more competitive.

==> figures/Fig-exp-CP.tex <==
\begin{figure*}[t]

\begin{minipage}[b]{.3\linewidth}
    \centering
    \subfloat[][]{\label{cartesian_det}\includegraphics[ width=0.985\linewidth]{images/Figure5_b.pdf}}
\end{minipage}
\hspace{-2.5pt}
\begin{minipage}[b]{.69\linewidth}
    \centering
    \subfloat[][]{\label{polar_det}\includegraphics[width=0.9\linewidth]{images/Figure5_a.pdf}}
    
    \subfloat[][]{\label{diff_dist}
    \small
    \begin{subtable}[h]{\textwidth}
        \centering
        \setlength{\tabcolsep}{4pt}
        \renewcommand{\arraystretch}{1.2}{
        \begin{tabular}{ll||ccc}
        \hline
        
        \hline
        \rowcolor{white}
        \textbf{Method} & \textbf{Coordinate} & \textbf{Near} & \textbf{Medium} & \textbf{Far} \\
        \hline
        DETR3D~\cite{wang2022detr3d} & Cartesian & 49.9/49.3 & 28.6/39.2 & 8.1/21.2 \\
        BEVFormer-S~\cite{li2022bevformer} & Cartesian & 54.2/53.5 & 31.7/41.3 & 9.5/21.9  \\
        PolarFormer-CC & Cartesian & 54.7/55.5 & 32.3/42.2 & 9.4/22.2\\
        \rowcolor[gray]{.9} 
        PolarFormer & Polar & \textbf{57.8/55.8} & \textbf{33.6/42.9} & \textbf{9.6/22.3}  \\
        \hline
        
        \hline
        \end{tabular}
        }
        \label{table:coordinate}
    \end{subtable}
    
    }
\end{minipage} %\par
\caption{
3D object detection in (a) Cartesian BEV {\em vs.} (b) Polar BEV, and (c) Performance comparison (mAP/NDS) at three distances (Near/Medium/Far). 
Red and green boxes show the same objects in different coordinates.
}
% \hspace{-10pt}
% \vspace{-0.3cm}
\label{fig:polarcardi}
\end{figure*}

==> figures/Fig-exp-feat_attn.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.52\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0 0.865cm 0 0}]{images/exp_feat_attn_a.pdf}
         \caption{}
         \label{fig:encoder_feat}
     \end{subfigure}
     \hspace{-5pt}
     \begin{subfigure}[b]{0.449\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0 -0.015cm 0 0}]{images/exp_feat_attn_b.pdf}
         \caption{}
         \label{fig:query_attn}
     \end{subfigure}
     \hfill
        \caption{Visualization of the output of the encoder as well as the attention generated by the query.}
        \label{fig:exp_feat_attn}
\end{figure}

==> figures/Fig-exp-vis.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \makebox[\textwidth][c]{\includegraphics[width=1.2\textwidth]{images/5.pdf}}
         \label{fig:4}
     \end{subfigure}
      \caption{Visualizations: Given multi-camera images, our method is dedicated to perform 3D object detection and BEV semantic segmentation.}
     \label{fig:supp_vis_3}
\end{figure}

==> figures/Fig-model_arch-attention.tex <==
\begin{figure}[t]
\begin{minipage}[]{0.49\linewidth}
\centering
\footnotesize
\setlength{\tabcolsep}{3.8pt}
\renewcommand{\arraystretch}{1.325}{
\begin{tabular}{ll||c||lll}
\hline

\hline
\textbf{Enc.} & \textbf{Dec.} & \textbf{Diff. res.} & \textbf{mAP}$\uparrow$ & \textbf{NDS}$\uparrow$ & \textbf{FPS}$\uparrow$\\
\hline
3 & 3 & \XSolidBrush & 38.8 & 45.4 &  1.6 \\
3 & 3 & \Checkmark & 38.6 & 45.2 &  1.8 \\
\cmidrule(lr){1-6}
3 & 6 & \XSolidBrush  & 38.2 & 44.6 &  1.6 \\
3 & 6 & \Checkmark  & 38.4 & 44.7 & 1.8 \\
\cmidrule(lr){1-6}
6 & 6 & \XSolidBrush & 37.9 & 44.8 &  1.4 \\
\rowcolor[gray]{.9} 
6 & 6 & \Checkmark & \textbf{39.6} & \textbf{45.8} &  1.7\\
\hline

\hline
\end{tabular}
}
% \vspace{1.75pt}
\captionof{table}{Ablation study on model architecture.}
\label{table:ablation_model_arch}
\end{minipage}
\begin{minipage}[]{.51\linewidth}
 \centering
 \includegraphics[height=3.8cm, width=0.95\linewidth]{images/exp_feat_attn_b.pdf}
 \caption{Multi-scale Polar BEV attention.}
 \label{fig:query_attn}
\end{minipage}
\end{figure}

==> figures/Fig-multi-scale_coord.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.445\textwidth}
\centering
\includegraphics[width=1\textwidth, trim={0 0.285cm 0 0}]{images/coord.pdf}
\caption{Cartesian and Polar coordinates.}
\label{fig:learning_targets}
\end{minipage}
\begin{minipage}[t]{0.545\textwidth}
\centering
\includegraphics[width=0.6\textwidth,trim={0cm 0cm 0 0cm}]{images/multiscale_1.pdf}
\hspace{-0.75cm}
\includegraphics[height=2.225cm, width=0.25\textwidth,trim={-5.175cm -2cm 0 0cm}]{images/multiscale_2.pdf} 
\hspace{-0.15cm}
\includegraphics[width=0.225\textwidth,trim={0cm 0cm 0 0cm}]{images/multiscale_3.pdf}
\caption{Multi-scale Polar BEV maps.}
\label{fig:multi-scale}
\end{minipage}
\end{figure}


==> figures/Fig1-teaser.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{images/teaser.pdf}
    \caption{
    Taking multi-camera images as input, the proposed \texttt{PolarFormer} model is designed particularly 
    for accurate 3D object detection
    in the Polar coordinate system.
    }
    \label{fig:teaser}
\end{figure}


==> figures/Fig2-pipeline.tex <==
\begin{figure}
    \centering
    % \vspace{-2mm}
    \begin{overpic}[width=1.02\textwidth]
    {images/pipeline.pdf}
    \put(43.0,31.0){\scriptsize \textbf{(a)}}
    \put(40.0,29.5){\scriptsize Cross-plane}
    \put(41.0,28.0){\scriptsize encoder}
    %
    \put(27,48.0){\scriptsize \textbf{(b)} Polar alignment module}
    %
    \put(62.0, 13.5){\scriptsize \textbf{(c)}}
    \put(59.5, 12.0){\scriptsize Polar BEV}
    \put(61.0, 10.5){\scriptsize encoder}
    \end{overpic}
    \caption{Schematic illustration of our proposed {\em PolarFormer} for multi-camera 3D object detection. 
    For each image captured by any camera view, our model first extracts the feature maps at multiple spatial scales. 
    Given such a feature map, the cross-plane encoder \textbf{(a)} then transforms all the feature columns to a set of Polar rays in a sequence-to-sequence manner via polar queries based cross-attention. The polar rays from all the cameras are subsequently processed by a Polar alignment module \textbf{(b)} to generate a structured multi-scale Polar BEV map, followed by further enhancement via interactions among different scales using a Polar BEV encoder \textbf{(c)}.
    At last, a specially designed Polar Head decodes multi-scale Polar BEV features for making final predictions in the Polar coordinate.}
    \label{fig:pipeline}
\end{figure}
